IDK-MRC: Unanswerable Questions for Indonesian Machine Reading Comprehension

Machine Reading Comprehension (MRC) has become one of the essential tasks in Natural Language Understanding (NLU) as it is often included in several NLU benchmarks (Liang et al., 2020; Wilie et al., 2020). However, most MRC datasets only have answerable question type, overlooking the importance of unanswerable questions. MRC models trained only on answerable questions will select the span that is most likely to be the answer, even when the answer does not actually exist in the given passage (Rajpurkar et al., 2018). This problem especially remains in medium- to low-resource languages like Indonesian. Existing Indonesian MRC datasets (Purwarianti et al., 2007; Clark et al., 2020) are still inadequate because of the small size and limited question types, i.e., they only cover answerable questions. To fill this gap, we build a new Indonesian MRC dataset called I(n)don'tKnow- MRC (IDK-MRC) by combining the automatic and manual unanswerable question generation to minimize the cost of manual dataset construction while maintaining the dataset quality. Combined with the existing answerable questions, IDK-MRC consists of more than 10K questions in total. Our analysis shows that our dataset significantly improves the performance of Indonesian MRC models, showing a large improvement for unanswerable questions.

==> tables/data_type_distribution.tex <==
\begin{table}[t!]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}lrrr@{}}
        \toprule
        \multicolumn{1}{c}{\textbf{Question Type}} & \textbf{M-Gen} & \multicolumn{1}{c}{\textbf{H-Filt}} & \multicolumn{1}{c}{\textbf{IDK-MRC}} \\ \midrule
        Negation & 15.84\% & 10.84\% & 9.95\% \\
        Antonym & 11.11\% & 16.06\% & 17.06\% \\
        Entity Swap & 49.17\% & 59.04\% & 27.73\% \\
        Question Tag Swap & 4.96\% & 3.61\% & 6.87\% \\
        Specific Condition & 4.02\% & 3.61\% & 20.85\% \\
        Other & 6.38\% & 6.83\% & 17.54\% \\ \midrule
        Noise (answerable) & 8.51\% & 0.00\% & 0.00\% \\ \bottomrule
    \end{tabular}%
    }
    \caption{The distribution of unanswerable question types of Model Gen (\textbf{M-Gen}), Model Gen + Human Filt (\textbf{H-Filt}), and \textbf{IDK-MRC} test set. The definition of each question type is described in Table \ref{tab:data-sample}.}
    \label{tab:type-stat}
\end{table}

==> tables/result_checklist_en.tex <==
\begin{table*}[t!]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{@{}lcccccccccccccccr@{\hskip3pt}l@{}}
        \toprule
        \multicolumn{1}{c}{\multirow{3}{*}{}} & \multicolumn{15}{c}{\textbf{Failure Rate}} & \multicolumn{2}{c}{\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Failure Cases Examples\\ with expected answer (A)\\ and model prediction (P)\end{tabular}}}} \\
        \multicolumn{1}{c}{} & \multicolumn{5}{c|}{\textbf{IndoBERT}} & \multicolumn{5}{c|}{\textbf{m-BERT}} & \multicolumn{5}{c}{\textbf{XLM-R}} & \multicolumn{2}{c}{} \\
        \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{TR}} & \multicolumn{1}{c}{\textbf{OR}} & \multicolumn{1}{c}{\textbf{MG}} & \multicolumn{1}{c}{\textbf{HF}} & \multicolumn{1}{c|}{\textbf{HA}} & \multicolumn{1}{c}{\textbf{TR}} & \multicolumn{1}{c}{\textbf{OR}} & \multicolumn{1}{c}{\textbf{MG}} & \multicolumn{1}{c}{\textbf{HF}} & \multicolumn{1}{c|}{\textbf{HA}} & \multicolumn{1}{c}{\textbf{TR}} & \multicolumn{1}{c}{\textbf{OR}} & \multicolumn{1}{c}{\textbf{MG}} & \multicolumn{1}{c}{\textbf{HF}} & \multicolumn{1}{c}{\textbf{HA}} & \multicolumn{2}{c}{} \\ \midrule
        \multirow{6}{*}{\rotatebox[origin=c]{90}{Negation}} & \multirow{3}{*}{0.4} & \multirow{3}{*}{100} & \multirow{3}{*}{\textbf{0}} & \multirow{3}{*}{2.3} & \multicolumn{1}{r|}{\multirow{3}{*}{6.7}} & \multirow{3}{*}{\textbf{0}} & \multirow{3}{*}{100} & \multirow{3}{*}{\textbf{0}} & \multirow{3}{*}{\textbf{0}} & \multicolumn{1}{r|}{\multirow{3}{*}{\textbf{0}}} & \multirow{3}{*}{\textbf{0}} & \multirow{3}{*}{100} & \multirow{3}{*}{\textbf{0}} & \multirow{3}{*}{\textbf{0}} & \multirow{3}{*}{0.3} & C: & Wikia was designed by James. \\
         &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  &  & Q: & What was not designed by James? \\
         &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  &  & A: & \texttt{{[}empty{]}} P: Wikia \\ \cmidrule(l){2-18} 
         & \multirow{3}{*}{\textbf{42.4}} & \multirow{3}{*}{100} & \multirow{3}{*}{84.4} & \multirow{3}{*}{100} & \multicolumn{1}{r|}{\multirow{3}{*}{99.8}} & \multirow{3}{*}{\textbf{46.3}} & \multirow{3}{*}{100} & \multirow{3}{*}{74.6} & \multirow{3}{*}{99.9} & \multicolumn{1}{r|}{\multirow{3}{*}{80.5}} & \multirow{3}{*}{59.3} & \multirow{3}{*}{100} & \multirow{3}{*}{84.1} & \multirow{3}{*}{94.7} & \multirow{3}{*}{\textbf{48.9}} & C: & Wikia is not chaired by Ali. \\
         &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  &  & Q: & Who is Wikia's chair? \\
         &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  &  & A: & \texttt{{[}empty{]}} P: Ali \\ \midrule
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Antonym}} & \multirow{3}{*}{\textbf{90.6}} & \multirow{3}{*}{100} & \multirow{3}{*}{100} & \multirow{3}{*}{100} & \multicolumn{1}{r|}{\multirow{3}{*}{98.3}} & \multirow{3}{*}{\textbf{57.7}} & \multirow{3}{*}{100} & \multirow{3}{*}{79.2} & \multirow{3}{*}{89.4} & \multicolumn{1}{r|}{\multirow{3}{*}{76.6}} & \multirow{3}{*}{74.2} & \multirow{3}{*}{100} & \multirow{3}{*}{90.4} & \multirow{3}{*}{90.2} & \multirow{3}{*}{\textbf{64.6}} & C: & Bia got the highest prize. \\
         &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  &  & Q: & Who got the lowest prize? \\
         &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  &  & A: & \texttt{{[}empty{]}} P: Bia \\ \midrule
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Ent Swp}} & \multirow{3}{*}{80.4} & \multirow{3}{*}{100} & \multirow{3}{*}{19.8} & \multirow{3}{*}{\textbf{2.6}} & \multicolumn{1}{r|}{\multirow{3}{*}{8.2}} & \multirow{3}{*}{17.4} & \multirow{3}{*}{100} & \multirow{3}{*}{0.7} & \multirow{3}{*}{\textbf{0.6}} & \multicolumn{1}{r|}{\multirow{3}{*}{2.1}} & \multirow{3}{*}{38.5} & \multirow{3}{*}{100} & \multirow{3}{*}{16.3} & \multirow{3}{*}{\textbf{8.2}} & \multirow{3}{*}{11.8} & C: & Dewi is the president of Cuba. \\
         &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  &  & Q: & Who is the president of Chile? \\
         &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  &  & A: & \texttt{{[}empty{]}} P: Dewi \\ \midrule
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Q Swp}} & \multirow{3}{*}{98.7} & \multirow{3}{*}{100} & \multirow{3}{*}{100} & \multirow{3}{*}{98.3} & \multicolumn{1}{r|}{\multirow{3}{*}{\textbf{79.3}}} & \multirow{3}{*}{87.4} & \multirow{3}{*}{100} & \multirow{3}{*}{87.8} & \multirow{3}{*}{95.6} & \multicolumn{1}{r|}{\multirow{3}{*}{\textbf{65.1}}} & \multirow{3}{*}{67.9} & \multirow{3}{*}{100} & \multirow{3}{*}{85.8} & \multirow{3}{*}{94.4} & \multirow{3}{*}{\textbf{49.4}} & C: & Anita was born in Israel. \\
         &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  &  & Q: & When was Anita born? \\
         &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  &  & A: & \texttt{{[}empty{]}} P: Israel \\ \midrule
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Unavbl C}} & \multirow{3}{*}{70.3} & \multirow{3}{*}{100} & \multirow{3}{*}{58.6} & \multirow{3}{*}{70.8} & \multicolumn{1}{r|}{\multirow{3}{*}{\textbf{23.8}}} & \multirow{3}{*}{66.1} & \multirow{3}{*}{100} & \multirow{3}{*}{25.1} & \multirow{3}{*}{44.6} & \multicolumn{1}{r|}{\multirow{3}{*}{\textbf{8.2}}} & \multirow{3}{*}{62.0} & \multirow{3}{*}{100} & \multirow{3}{*}{43.4} & \multirow{3}{*}{51.1} & \multirow{3}{*}{\textbf{18.3}} & C: & Roy is a president. \\
         &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  &  & Q: & Who is the retired president? \\
         &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  &  & A: & \texttt{{[}empty{]}} P: Roy \\ \midrule
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Other}} & \multirow{3}{*}{85.6} & \multirow{3}{*}{100} & \multirow{3}{*}{74.5} & \multirow{3}{*}{59.7} & \multicolumn{1}{r|}{\multirow{3}{*}{\textbf{22.5}}} & \multirow{3}{*}{31.1} & \multirow{3}{*}{100} & \multirow{3}{*}{42.3} & \multirow{3}{*}{53.0} & \multicolumn{1}{r|}{\multirow{3}{*}{\textbf{24.3}}} & \multirow{3}{*}{47.9} & \multirow{3}{*}{100} & \multirow{3}{*}{34.6} & \multirow{3}{*}{22.1} & \multirow{3}{*}{\textbf{9.3}} & C: & Sheila is Rudy's fan. \\
         &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  &  & Q: & Who is Rudy's friend? \\
         &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  & \multicolumn{1}{r|}{} &  &  &  &  &  & A: & \texttt{{[}empty{]}} P: Sheila \\ \midrule
        \multicolumn{1}{c}{\textbf{}} & 74.5 & 100 & 65.9 & 63.8 & \multicolumn{1}{r|}{\textbf{47.6}} & 47.1 & 100 & 45.4 & 55.5 & \multicolumn{1}{r|}{\textbf{36.1}} & 53.4 & 100 & 52.1 & 52.2 & \textbf{29.7} & \multicolumn{1}{l}{} &  \\ \bottomrule
    \end{tabular}%
    }
    \caption{The failure rate on all unanswerable question types tested using the CheckList tool \cite{ribeiro-etal-2020-beyond}. The scores are the mean over 5 runs with different random seeds (lower score is better). The \textbf{last row} denotes the \textbf{macro average} of all unanswerability types. For table presentation effectiveness, the test case examples are shown in English. The real test cases are in Indonesian. \textbf{TR}: Trans, \textbf{OR}: Orig, \textbf{MG}: M-Gen, \textbf{HF}: H-Filt, \textbf{HA}: H-Add.}
    \label{tab:checklist}
\end{table*}
